A Metric Learning Reality Check

Deep metric learning papers from the past four years have consistently claimed great advances in accuracy, often more than doubling the performance of decade-old methods. In this paper, we take a closer look at the field to see if this is actually true. We find flaws in the experimental methodology of numerous metric learning papers, and show that the actual improvements over time have been marginal at best.

==> hidden_citations.tex <==


Contrastive*,
Triplet*,
Semihard Mining*,
N-Pairs \cite{sohn2016improved},
Histogram \cite{ustinova2016learning},
Lifted Structure \cite{oh2016deep},
HDC \cite{yuan2017hard},
Angular \cite{wang2017deep},
Spectral \cite{law2017deep},
Clustering \cite{oh2017deep},
ProxyNCA \cite{movshovitz2017no},
Margin loss \cite{wu2017sampling},
DAML \cite{duan2018deep},
DVML \cite{lin2018deep},
Normalized Softmax \cite{zhai2018classification},
HTL \cite{ge2018deep},
Asymmetric ML \cite{xu2019deep},
DeML \cite{chen2019hybrid},
HDML \cite{zheng2019hardness},
Stochastic Hard Mining \cite{suh2019stochastic},
HORDE \cite{jacob2019metric},
Multi Similarity \cite{wang2019multi},
Ranked List \cite{wang2019ranked},
SoftTriple \cite{qian2019softtriple},
Divide and Conquer \cite{sanakoyeu2019divide},
MIC \cite{roth2019mic},
FastAP \cite{cakir2019deep},
Tuplet Margin Loss \cite{Yu_2019_ICCV},
Circle Loss \cite{sun2020circle},
Proxy Anchor \cite{kim2020proxy},
EPSHN \cite{xuan2020improved}


==> related.tex <==


\sjb{This is well phrased, but since it's short, I wonder if it should just be a subsection in the intro, e.g., right before Contributions.}
